An Accurate Globally Conservative Subdomain Discontinuous Least-squares Scheme for Solving Neutron Transport Problems

In this work, we present a subdomain discontinuous least-squares (SDLS) scheme for neutronics problems. Least-squares (LS) methods are known to be inaccurate for problems with sharp total-cross section interfaces. In addition, the least-squares scheme is known not to be globally conservative in heterogeneous problems. In problems where global conservation is important, e.g. k-eigenvalue problems, conservative treatment must be applied. We, in this study, proposed a SDLS method that retains global conservation. Such a method resembles the LS formulation in each subdomain without material interface and differs from LS in that an additional least-squares interface term appears for each interface. Scalar flux is continuous in each subdomain with continuous finite element method (CFEM) while discontinuous on interfaces for every pair of contiguous subdomains. SDLS numerical results are compared with those obtained from other numerical methods with test problems having material interfaces. High accuracy of scalar flux in fixed-source problems and $k_\mathrm{eff}$ in eigenvalue problems are demonstrated.

==> mybibfile.tex <==

@comment{This file has been generated by Pybliographer}


@Book{book,
	Author         = {{Ian M. Babbelbox}},
	Title          = {Zen and the {A}rt of {LWR} {M}aintenance},
	Publisher      = {Wiley Coyote \& Sons},
	Address        = {Palookaville, USA},
	month          = mar,
	year           = 1998
}

@mastersthesis{thesis,
	author = {Zheng, Weixiong},
	title = {Physics-Based Uncertainty Quantification for ZrHx Thermal	Scattering Law},
	school = {Texas A\&M University},
	month = {December},
	year = {2013}
}
@article{Morel:2000vh,
author = {Morel, J. E.},
title = {{Diffusion-limit asymptotics of the transport equation, the P$_{1/3}$ equations, and two flux-limited diffusion theories}},
journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
year = {2000},
volume = {65},
number = {5},
pages = {769--778}
}
@article{adams2001discontinuous,
  title={Discontinuous finite element transport solutions in thick diffusive problems},
  author={Adams, Marvin L},
  journal={Nuclear Science and Engineering},
  volume={137},
  number={3},
  pages={298--333},
  year={2001},
  publisher={American Nuclear Society}
}

@article{sanchez-transport,
	title={A Review of Neutron Transport Approximations},
	author={R. Sanchez and N. J. McCormick},
	journal={Nuclear Science and Engineering},
	volume={80},
	pages={481--535},
	year={1982},
	publisher={American Nuclear Society}
}

@ARTICLE{laboure:2016,
   author = {{Laboure}, V.~M. and {McClarren}, R.~G. and {Wang}, Y.},
    title = "{Globally Conservative, Hybrid Self-Adjoint Angular Flux and Least-Squares Method Compatible with Void}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1605.05388},
 primaryClass = "physics.comp-ph",
 keywords = {Physics - Computational Physics},
     year = 2016,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160505388L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@techreport{zheng-inl,
	Author = {Weixiong Zheng and Yaqi Wang and Mark DeHart},
	Institution = {Idaho National Laboratory},
	Number = {INL/EXT-16-39793},
	Title = {Multiscale Capability in Rattlesnake using Contiguous Discontinuous Discretization of Self-Adjoint Angular Flux Equation},
	Year = {2016}}

@article{bicgstab,
	author = {H. A. van der Vorst},
	title = {Bi-CGSTAB: A Fast and Smoothly Converging Variant of Bi-CG for the Solution of Nonsymmetric Linear Systems},
	journal = {SIAM Journal on Scientific and Statistical Computing},
	volume = {13},
	number = {2},
	pages = {631-644},
	year = {1992}
}

@article{Olson:2000vq,
author = {Olson, G. L. and Auer, L. H. and Hall, M. L.},
title = {{Diffusion, P$_1$, and other approximate forms of radiation transport}},
journal = {Journal of Quantitative Spectroscopy and Radiative Transfer},
year = {2000},
volume = {64},
number = {6},
pages = {619--634}
}

@article{yaqi_invite,
	author = {Y. Wang and S. Schunert and M. DeHart and R. Matineau and W. Zheng},
	title = {{Hybrid P$_N$-S$_N$\ With Lagrange Multiplier and Upwinding for the Multiscale Transport Capability in Rattlesnake}},
	year = {2016},
	journal = {Progress in Nuclear Energy (submitted on Sept. 2016)}
}

@article{zheng_invite,
	author = {Weixiong Zheng and Ryan G. McClarren},
	title = {{Accurate Least-Squares PN Scaling based on Problem Optical Thickness for solving Neutron Transport Problems}},
	year = {2016},
	journal = {Progress in Nuclear Energy (submitted on Sept. 2016)}
}

@article{adams_iron_water,
author = {Chris L. Castrianni and Marvin L. Adams},
title={{A Nonlinear Corner-Balance Spatial Discretization for Transport on Arbitrary Grids}},
journal={Nuclear Science and Engineering},
volume={128},
year={1998},
number={3},
pages={278--296}
}

@article{morel_saaf,
	author = {Jim E. Morel and J. M. McGhee},
	title={{A Self-Adjoint Angular Flux Equation}},
	journal={Nuclear Science and Engineering},
	volume={132},
	year={1999},
	number={3},
	pages={312--325}
}

@ARTICLE{manteuffel_lspn_scaling,
	author = {T. A. Manteuffel and K. J. Ressel},
	title = {{Least-Squares Finite-Element Solution of the Nuetron Transport Equation in Diffusive Regimes}},
	journal = {SIAM J. Numer. Anal},
	volume = {35},
	number = {2},
	year = {1998},
	pages = {806-835},
}

@article{varin_lspn,
	Author = {Varin, E. and Samba, G.},
	Journal = {Nuclear Science and Engineering},
	Keywords = {lspn},
	Pages = {167--183},
	Title = {{Spherical Harmonics Finite Element Transport Equation Solution Using a Least-Square Approach}},
	Volume = {151},
	Year = {2005}}

@phdthesis{gesh_dissertation,
	title    = {Finite Element Methods for Second Order Forms of the Transport Equation},
	school   = {Texas A\&M University},
	author   = {C. J. Gesh},
	type     = {{PhD} dissertation},
	year     = {1999}
}

@inproceedings{gesh_mc,
	author={C. J. Gesh and M. L. Adams},
	title={{Finite Element Solutions of Second-order Forms of the Transport Equation at the Interface Between Diffusive and Non-Diffusive Regions}},
	booktitle={M\&C 2001},
	note={Salt Lake City, Utah, United States},
	year={2001}
}

@inproceedings{bochev-ls,
	author={P. Bochev and M. Gunzburger},
	title={{Least-squares finite element methods}},
	booktitle={ICM2006},
	note={Madrid, Spain},
	year={2006}
}

@article{yaqi_void,
	Author = {Y. Wang and H. Zhang and R. C. Martineau},
	Journal = {Nuclear Science and Engineering},
	Number = {2},
	Pages = {201--225},
	Title = {{Diffusion Acceleration Schemes for Self-Adjoint Angular Flux Formulation with a Void Treatment}},
	Volume = {176},
	Year = {2014}}

@article{runchang,
	author = {Runchang Lin},
	title = {{Discontinuous Discretization for Least-Squares Formulation of Singularity Perturbed Reaction-Diffusion Problems in One and Two Dimensions}},
	journal = {SIAM J. NUMER. ANAL},
	volume = {47},
	number = {1},
	pages = {89--108},
	year = {2008}
}

@article{morel_saai,

title = "Spatial discretizations for self-adjoint forms of the radiative transfer equations ",

journal = "Journal of Computational Physics ",

volume = "214",

number = "1",

pages = "12 - 40",

year = "2006",

note = "",

issn = "0021-9991",

doi = "http://dx.doi.org/10.1016/j.jcp.2005.09.017",

url = "http://www.sciencedirect.com/science/article/pii/S0021999105004213",

author = "Jim E. Morel and B. Todd Adams and Taewan Noh and John M. McGhee and Thomas M. Evans and Todd J. Urbatsch",

keywords = "Thermal radiation transport",

keywords = "Self-adjoint equations",

keywords = "Finite-elements "

}





@article{McClarren:2011ga,
author = {McClarren, R. G},
title = {{Theoretical Aspects of the Simplified P$_n$ Equations}},
journal = {Transport Theory and Statistical Physics},
year = {2011},
volume = {39},
number = {2-4},
pages = {73--109}
}


@article{McClarren:2008hu,
author = {McClarren, Ryan G and Holloway, James Paul and Brunner, Thomas A},
title = {{On solutions to the P$_n$ equations for thermal radiative transfer}},
journal = {Journal of Computational Physics},
year = {2008},
volume = {227},
number = {5},
pages = {2864--2885},
month = feb
}

@article{McClarren:2010de,
author = {McClarren, Ryan G and Hauck, Cory D},
title = {{Robust and accurate filtered spherical harmonics expansions for radiative transfer}},
journal = {Journal of Computational Physics},
year = {2010},
volume = {229},
number = {16},
pages = {5597--5614},
month = aug
}


@article{Hansen:2015jq,
author = {Hansen, Jon and Peterson, Jacob and Morel, Jim and Ragusa, J. E.an and Wang, Yaqi},
title = {{A Least-Squares Transport Equation Compatible with Voids}},
journal = {Journal of Computational and Theoretical Transport},
year = {2015},
volume = {43},
number = {1-7},
pages = {374--401},
month = feb
}

@article{cory_hauck_closures,
author = {C. Kristopher Garrett and Cory D. Hauck},
title = {{A Comparison of Moment Closures for Linear Kinetic Transport Equations: The Line Source Benchmark}},
journal = {Transport Theory and Statistical Physics},
volume = {42},
number = {6-7},
pages = {203--235},
year = {2013},
doi = {10.1080/00411450.2014.910226}
}

@article{ppn,
author = {Cory D. Hauck and Ryan G. McClarren},
title = {{Positive P$_N$ Closures}},
journal = {SIAM Journal on Scientific Computing},
volume = {32},
number = {5},
pages = {2603--2626},
year = {2010},
doi = {10.1137/090764918}
}

@article{cockburn_ldg,
	author = {Bernardo Cockburn and Chi-Wang Shu},
	title = {{The Local Discontinuous Galerkin finite element method for convection–-diffusion systems}},
	journal = {SIAM J. Numer. Anal.},
	volume = {35},
	pages = {2440--2463},
	year = {1998},
	doi = {10.1137/090764918}
}

@Misc{website,
	Title          = {Research {I}nstitute of {N}uclear {E}ngineering,
	{U}niversity of {F}ukui},
	HowPublished   = {Available online},
	url            = {https://urldefense.proofpoint.com/v2/url?u=http-3A__www.rine.u-2Dfukui.ac.J&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=2Z0xaU4WXDOrEVEJTkd4unZ5_8S-YvAgaSVdlMnM-TU&e= . P./english/index.html},
	year           = 2013
}


@book{santner2003design,
	author = {Santner, T. J. and Williams, B. J. and Notz, W.},
	title = {{The {D}esign and Analysis of Computer Experiments}},
	publisher = {Springer},
	address = {New York, NY},
	year = {2003},
	series = {Springer Series in Statistics}
}


@article{Slaggie,
	Author = {E. L. Slaggie},
	Date-Added = {1967-11-29 15:01:35 -0500},
	Date-Modified = {1967-11-29 15:01:35 -0500},
	Journal = {J. Phys. Chem. Solids},
	Keywords = {SN},
	Pages = {923--934},
	Title = {{Central {F}orce Lattice Dynamical Model for Zirconium Hydride}},
	Volume = {29},
	Year = {1968}}

@article{pomraning_saaf,
    Author = {G. C. Pomraning and M. Clark, Jr},
    Journal = {Nuclear Science and Engineering},
    Year = {1963},
    Number = {2},
    Volume = {16},
    Pages = {155-164},
    Title = {{The Variational Method Applied to the Monoenergetic Boltzmann Equation. Part II}}
}

@techreport{IKE,
	Author = {Mattes, M. and Keinert, J.},
	Date-Added = {2010-01-15 14:53:00 -0500},
	Date-Modified = {2010-01-15 14:53:00 -0500},
	Institution = {Institue for Nuclear Technology and EneR. G.y System (IKE)-University of Stuttgart},
	Number = {INDC(NDS)-0470},
	Title = {{Thermal Netron Scattering Data for the Moderator Materials H$_2$O, D$_2$O and ZrH$_x$\, in ENDF-$6$ Format and as ACE Library for MCNP(X) Code}},
	Year = {2005}}

@techreport{triga,
	Author = {Texas A\&M University, Nuclear Science Center},
	Date-Added = {2010-01-15 14:53:00 -0500},
	Date-Modified = {2010-01-15 14:53:00 -0500},
	Institution = {Nuclear Science Center, Texas A\&M University},
	Number = {05000128},
	Title = {{Safety Analysis Report}},
	Year = {2011}}

@inproceedings{Badea,
	Author = {Badea, M. D. R. and Broeders, C. H. M.},
	Date-Added = {1967-11-29 15:01:35 -0500},
	Date-Modified = {1967-11-29 15:01:35 -0500},
	Booktitle = {International Conference on Nuclear Data for Science and Technology 2007},
	Title = {{On the Impact of Phonon Spectrum Shifts of the Hydrogen Binding in ZrH}},
	Number = {242},
	DOI = {10.1051/ndata:07681},
	Year = {2008}}

@inproceedings{weixiong,
	Author = {Zheng, W. and McClarren, R. G.},
	Booktitle = {{ANS Winter Meeting 2013}},
	Title = {{Physics-Based Uncertainty Quantification for ZrHx Thermal Scattering Law}},
	Pages = {743--745},
	Volume = {109},
	Number = {1},
	OR. G.anization   = {ANS},
	note           = {Washington, D.C., November 10 - 14},
	Year = {2013}}

@inproceedings{yaqi-rattlesnake,
	Author = {Frederick N. Gleicher and Yaqi Wang and Derek Gaston and Richard C. Martineau},
	Booktitle = {{Transactions of American Nuclear Society}},
	Title = {{The Method of Manufactured Solutions for RattleSnake, A SN Radiation Transport Solver Inside the MOOSE Framework}},
	Pages = {372--374},
	Volume = {106},
	Number = {1},
	OR. G.anization   = {ANS},
	Year = {2012}}

@inproceedings{zheng_l1sn,
	Author = {Zheng, W. and McClarren, R. G.},
	Booktitle = {{ANS Winter Meeting 2015}},
	Title = {{Non-oscillatory Reweighted Least Square Finite Element Method for S$_N$\ Transport}},
	Pages = {688--691},
	Volume = {113},
	Number = {1},
	OR. G.anization   = {ANS},
	note           = {Washington, D.C.},
	Year = {2015}}

@phdthesis{zheng_dissertation,
	title    = {Least-Squares and Other Residual Based Techniques for Radiation Transport Calculations},
	school   = {Texas A\&M University},
	author   = {Weixiong Zheng},
	type     = {{PhD} dissertation},
	year     = {2016}
}

@inproceedings{zheng_l1pn,
	Author = {Zheng, W. and McClarren, R. G.},
	Booktitle = {{ANS Winter Meeting 2015}},
	Title = {{Non-oscillatory Reweighted Least Square Finite Element for Solving $P_N$\ Transport}},
	Pages = {692--695},
	Volume = {113},
	Number = {1},
	OR. G.anization   = {ANS},
	note           = {Washington, D.C.},
	Year = {2015}}

@inproceedings{taylor_ans12,
	Author = {McClarren, R. G. and Lane, T. K.},
	Booktitle = {{ANS Winter Meeting 2012}},
	Title = {{A Flux-Limited Diffusion Method for Simulating Radiative Shocks}},
	Pages = {557--559},
	Volume = {107},
	ORGanization   = {ANS},
	note           = {San Diego, CA, November},
	Year = {2012}}
@article{Mathews:1999uv,
author = {Mathews, Kirk A},
title = {{On the propagation of rays in discrete ordinates}},
journal = {Nuclear science and engineering},
year = {1999},
volume = {132},
number = {2},
pages = {155--180}
}

@article{Morel:2003vt,
author = {Morel, J. E. and Wareing, T. A. and Lowrie, R. B. and Parsons, D. K.},
title = {{Analysis of ray-effect mitigation techniques}},
journal = {Nuclear science and engineering},
year = {2003},
volume = {144},
number = {1}
}

@inproceedings{vincent-physor16,
	Author = {Vincent M. Laboure and Y. Wang and M. D. DeHart},
	Booktitle = {{PHYSOR 2016}},
	Title = {Least-squares PN Formulation of the Transport Equation Using Self-Adjoint Angular Flux Consistent Boundary Conditions},
	note           = {Sun Valley, ID, May 01 - 05},
	Year = {2016}}

@inproceedings{physor,
	Author = {Zheng, W. and McClarren, R. G.},
	Date-Added = {1967-11-29 15:01:35 -0500},
	Date-Modified = {1967-11-29 15:01:35 -0500},
	Booktitle = {{PHYSOR 2014 International Conference}},
	Title = {{Effective Physics-Based Uncertainty Quantification for ZrHx Thermal Neutron Scattering in TRIGA Reactors}},
	Pages = {743--745},
	Volume = {109},
	Number = {1},
	OR. G.anization   = {PHYSOR},
	note           = {Kyoto, Japan, September 28 - October 3},
	Year = {2014}}
	
@inproceedings{yaqi_physor16,
	Author = {S. Schunert and Y. Wang and M. D. DeHart and R. C. Martineau},
	Booktitle = {{PHYSOR 2016}},
	Title = {{Hybrid P$_N$-S$_N$\ Calculations with SAAF for the Multiscale Transport Capability in Rattlesnake}},
	OR. G.anization   = {PHYSOR},
	note           = {Sun Valley, ID, May 01 - 05},
	Year = {2016}}

@article{Grad:1949wi,
author = {Grad, Harold},
title = {{On the kinetic theory of rarefied gases}},
journal = {Communications on Pure and Applied Mathematics},
year = {1949},
volume = {2},
number = {4},
pages = {331--407}
}
@book{markowich2012semiconductor,
  title={Semiconductor Equations},
  author={Markowich, P. A. and Ringhofer, C. A. and Schmeiser, C.},
  isbn={9783709169612},
  url={https://urldefense.proofpoint.com/v2/url?u=https-3A__books.google.com_books-3Fid-3DnCr7CAAAQBAJ&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=5kz8cdvtmD5q5DJ_rVdid8dr6PSOMWzHUQiuF8PVC04&e= },
  year={2012},
  publisher={Springer Vienna}
}


@book{pomraning1973equations,
  title={The Equations of Radiation Hydrodynamics},
  author={Pomraning, G.C.},
  isbn={9780486445991},
  lccn={2005051881},
  series={Dover books on physics},
  url={https://urldefense.proofpoint.com/v2/url?u=https-3A__books.google.com_books-3Fid-3DEFbpgt-2DRlh8C&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=O1ITuhCUU7t4hMtI7iyr-Ocub4yGj35D6vz2SB8Rfuk&e= },
  year={1973},
  publisher={Dover Publications}
}

@article{Harling,
	Author = {Couch, J. G. and Harling, O. K. and Clune, L. C.},
	Date-Added = {1967-11-29 15:01:35 -0500},
	Date-Modified = {1967-11-29 15:01:35 -0500},
	Journal = {Physical Review B},
	Keywords = {SN},
	Pages = {923--934},
	Title = {{Structure in the Neutron Scattering Spectra of Zirconium Hydride}},
	Volume = {4},
	Number={8},
	Year = {1971}}

@book{glasstone,
	Author = {Bell, G. I. and Glasstone, S.},
	Title = {Nuclear Reactor Theory},
	Edition = {3rd},
	Publisher = {Krieger Pub Co},
	Year = {1985},
	Address = {Princeton, NJ}
}

@book{msa,
	title={{Mathematical Statistics with Applications}},
	author={Wackerly, D. D. and Mendenhall, W. and Scheaffer, R. L.},
	isbn={9780495385080},
	lccn={2007922554},
	year={2008},
	Edition = {7th},
	address={Belmont, CA},
	publisher={Cengage Learning Inc.}
}

@book{numerical,
	title={{Numerical Analysis: Mathematics of Scientific Computing}},
	author={D. R. Kincaid and E. W. Cheney},
	isbn={9780534389055},
	year={2001},
	Edition = {3th},
	address={Belmont, CA},
	publisher={Cengage Learning Inc.}
}

@techreport{Macf,
	Author = {MacFarlane, R. E.},
	Date-Added = {2010-01-15 14:53:00 -0500},
	Date-Modified = {2010-01-15 14:53:00 -0500},
	Institution = {Los Alamos National Laboratory},
	Number = {LA-12639-MS(ENDF 356)},
	Title = {{New Thermal Neutron Scattering Files for ENDF/B-VI$,$ Release 2}},
	Address = {Los Alamos, NM},
	Year = {1994}}

@article{fpn_radice,
	title = "A new spherical harmonics scheme for multi-dimensional radiation transport I. Static matter configurations ",
	journal = "Journal of Computational Physics ",
	volume = "242",
	number = "",
	pages = "648 - 669",
	year = "2013",
	note = "",
	issn = "0021-9991",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.jcp.2013.01.048",
	author = "David Radice and Ernazar Abdikamalov and Luciano Rezzolla and Christian D. Ott"}



@techreport{olson_report,
	Author = {Gordon L. Olson},
	Institution = {Los Alamos National Laboratory},
	Number = {LA-UR-12-22927},
	Title = {{Spherical Harmonic Solutions of the Radiation Transport Equation Using Angle-dependent Artificial
Scattering to Decrease Oscillations}},
	Address = {Los Alamos, NM},
	Year = {2012}}

@techreport{NJOY,
	Author = {MacFarlane, R. E. and Muir, D. W.},
	Date-Added = {2010-01-15 14:53:00 -0500},
	Date-Modified = {2010-01-15 14:53:00 -0500},
	Institution = {Los Alamos National Laboratory},
	Number = {LA-12740-M},
	Title = {{The NJOY Nuclear Data Processing System Version 91}},
	Year = {1994}}

@ARTICLE{Malik,
	author = {Malik, S. S. and Rorer, D. C. and Brunhart, G.},
	title = {{Optical-Phonon Structure and Precision Neutron Total Cross Section
	Measurements of Zirconium Hydride}},
	journal = {J. Phys. F: Met. Phys},
	year = {1984},
	volume = {14},
	pages = {73--81},
	date-added = {1983-8-1 15:01:35 -0500},
	date-modified = {1983-8-1 15:01:35 -0500},
	keywords = {SN}
}

@article{evans,
	title = {{Neutron-Scattering Study of the Impulse Approximation in ${\mathrm{ZrH}}_{2}$}},
	author = {Evans, A. C. and Timms, D. N. and Mayers, J. and Bennington, S. M.},
	journal = {Phys. Rev. B},
	volume = {53},
	issue = {6},
	pages = {3023--3031},
	year = {1996},
	month = {Feb.},
	doi = {10.1103/PhysRevB.53.3023},
	url = {https://urldefense.proofpoint.com/v2/url?u=http-3A__link.aps.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=G_Iy47ibdx4fTTFONVxYMsMUhnVO2Z8FyyQ2hTzlmeU&e= . G./doi/10.1103/PhysRevB.53.3023},
	publisher = {American Physical Society}
}

@ARTICLE{mck, 
	author={McKinny, K. S. and Anderson, T. R. and Johnson, N. H.}, 
	journal={Nuclear Science, IEEE Transactions on}, 
	title={{Optimization of Coating in Boron-10 Lined Proportional Counters}}, 
	year={2013}, 
	volume={60}, 
	number={2}, 
	pages={860-863}, 
	keywords={Monte Carlo methods;helium-3 counters;neutron detection;radiation monitoring;B;B-10 coating formulation;GE Reuter-Stokes;Helium-3 gas;MCNP modeling;boron-10 lined proportional counters;coating optimization;experimental data;individual detector;maximize sensitivity;moderator conήgurations;moderator design;neutron detection;optimal coating thickness;radiation portal monitors;thermal neutron ήeld;Coatings;Detectors;Monitoring;Neutrons;Portals;Radiation detectors;Sensitivity;Boron-10 (B-10) proportional counter;neutron detector;radiation portal monitor}, 
	doi={10.1109/TNS.2012.2224125}, 
	ISSN={0018-9499},}

@misc{mathematica,
	author = {Weisstein, E. W.},
	title = {{ANOVA}},
	howpublished = "\url{https://urldefense.proofpoint.com/v2/url?u=http-3A__mathworld.wolfram.com_ANOVA.html&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=PophkYbJcYoIzYPZT3ztx7W5QiKfWUhGzoTWx6yYq6o&e= }",
	year = {2008}, 
	note = "[Online; accessed 10-Oct.-2013]"
}

@misc{anova1,
	author = {The MathWorks Inc.},
	title = {{anova1,~one-way analysis of variance}},
	howpublished = "\url{https://urldefense.proofpoint.com/v2/url?u=http-3A__www.mathworks.com_help_stats_anova1.html&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=G8CRYPomQlIAhSrlaaHR9fQ2q5INMRCA7jLQI0G1O2I&e= }",
	note = "[Online; accessed 10-Oct.-2013]"
}

@misc{wikianova,
	author = {Wikipedia},
	title = {{Analysis of Variance --- {W}ikipedia{,} The Free Encyclopedia}},
	howpublished = "\url{https://urldefense.proofpoint.com/v2/url?u=http-3A__en.wikipedia.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=IyQb2O080OwHwr2sfCKjJzE6nFpFg0QKMVGFk3M1uwY&e= . G./wiki/Analysis_of_variance}",
	note = "[Online; accessed 9-Oct.-2013]"
}

@misc{data,
	title = {ENDF: Evaluated Nuclear Data File},
	url = {https://urldefense.proofpoint.com/v2/url?u=http-3A__www-2Dnds.iaea.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=8EXdyR0MRcojpTNjybBIrx8uNfjey6n8K2kmegbCG9Y&e= . G./endf/}}

@book{malick,
	author = {Denison, David G. T. and Holmes, Christopher C. and Mallick, Bani K. and Smith, Adrian F. M.},
	citeulike-article-id = {3872876},
	citeulike-linkout-0 = {https://urldefense.proofpoint.com/v2/url?u=http-3A__www.wiley.com_WileyCDA_WileyTitle_productCd-2D0471490369-2CdescCd-2DtableOfContents.html&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=OK0nFT2KaaAmBSl4vxxUKknMb30KFXpsDamSZCwdink&e= },
	keywords = {bayesian\_regression, nonparametric},
	posted-at = {2009-01-10 09:02:01},
	priority = {2},
	publisher = {Wiley},
	title = {{Bayesian Methods for Nonlinear Classification and Regression}},
	url = {https://urldefense.proofpoint.com/v2/url?u=http-3A__www.wiley.com_WileyCDA_WileyTitle_productCd-2D0471490369-2CdescCd-2DtableOfContents.html&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=OK0nFT2KaaAmBSl4vxxUKknMb30KFXpsDamSZCwdink&e= },
	year = {2002}
}

@article{stripbmars,
	title = "A calibration and data assimilation method using the Bayesian \{MARS\} emulator ",
	journal = "Annals of Nuclear EneR. G.y ",
	volume = "52",
	number = "0",
	pages = "103 - 112",
	year = "2013",
	note = "Nuclear Reactor Safety Simulation and Uncertainty Analysis ",
	issn = "0306-4549",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.anucene.2012.08.025",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__www.sciencedirect.com_science_article_pii_S0306454912003453&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=zGrUjDUkbL6F1avYIV294xSD_Nlf7LxkWFmcCh1nBaE&e= ",
	author = "H.F. Stripling and R. G. McClarren and C.C. Kuranz and M.J. Grosskopf and E. Rutter and B.R. Torralva",
	keywords = "Calibration",
	keywords = "Uncertainty quantification",
	keywords = "Predictive science",
	keywords = "Bayesian \{MARS\} "
}

@phdthesis{mccdissertation,
	title    = {{Spherical Harmonics Method for Thermal Radiation Transport}},
	school   = {University of Michigan},
	author   = {McClarren, Ryan G.},
	year     = {2007}, %other attributes omitted
}

@phdthesis{josh-quad,
	title    = {AN ADAPTIVE ANGULAR DISCRETIZATION METHOD FOR NEUTRAL-PARTICLE TRANSPORT IN THREE-DIMENSIONAL GEOMETRIES},
	school   = {Texas A\&M University},
	author   = {J. J. Jarrell},
	year     = {2010}, %other attributes omitted
}

@phdthesis{yaqi_dissertation,
	title    = {{Adaptive Mesh Refinement SOlution Techniques for the MUltigroup S$_N$\ Transport Equation Using a Higher-order Discontinuous Finite Element Method}},
	school   = {Texas A\&M University},
	author   = {Yaqi Wang},
	year     = {2009}, %other attributes omitted
}

@phdthesis{yunhuang_dissertation,
	title    = {{Even-parity S$_N$\ Adjoint Method Including SP$_N$\ Model Error and Iterative Efficiency}},
	school   = {Texas A\&M University},
	author   = {Yunhuang Zhang},
	year     = {2014}, %other attributes omitted
}

@article{brunner_2d_pn,
	title = "Two-dimensional time dependent {R}iemann solvers for neutron transport ",
	journal = "Journal of Computational Physics ",
	volume = "210",
	number = "1",
	pages = "386 - 399",
	year = "2005",
	note = "",
	issn = "0021-9991",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.jcp.2005.04.011",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__www.sciencedirect.com_science_article_pii_S0021999105002275&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Cp_ds5KNuvXxLRwTdv52FK60YlVIfLtS5LRzurpBe44&e= ",
	author = "Thomas A. Brunner and James Paul Holloway",
	keywords = "Riemann solvers",
	keywords = "Time dependent transport",
	keywords = "Spherical harmonics",
	keywords = "Finite methods",
	keywords = "Radiative transfer "
}

@article{pie,
	added-at = {2013-10-25T00:00:00.000+0200},
	author = {McClarren, Ryan G. and Ryu, Duchwan and Drake, R. Paul and Grosskopf, Michael and Bingham, Derek and Chou, Chuan-Chih and Fryxell, Bruce and van der Holst, Bart and Holloway, James Paul and Kuranz, Carolyn C. and Mallick, Bani K. and Rutter, Erica and Torralva, Ben R.},
	biburl = {https://urldefense.proofpoint.com/v2/url?u=http-3A__www.bibsonomy.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=NmaXsROWGrveWnaD1W3aIMA-bf3Q80yByawX-JcgDy8&e= . G./bibtex/2747960f429b314a8e493f5af93243023/dblp},
	ee = {https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.ress.2010.08.012},
	interhash = {eb8ecd5a6b8e6ee83445aeb0cfd8e086},
	intrahash = {747960f429b314a8e493f5af93243023},
	journal = {Rel. Eng. \& Sys. Safety},
	keywords = {dblp},
	number = 9,
	pages = {1194-1207},
	timestamp = {2013-10-25T00:00:00.000+0200},
	title = {A physics informed emulator for laser-driven radiating shock simulations.},
	url = {https://urldefense.proofpoint.com/v2/url?u=http-3A__dblp.uni-2Dtrier.de_db_journals_ress_ress96.html-23McClarrenRDGBCFHHKMRT11&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=tB7VenfqBVcXu3I_6eZU8isyzXHXnepDTjcbsxIfVrE&e= },
	volume = 96,
	year = 2011
}

@article{friedman1991,
	author = "Friedman, J. E.rome H.",
	doi = "10.1214/aos/1176347963",
	fjournal = "The Annals of Statistics",
	journal = "Ann. Statist.",
	month = "03",
	number = "1",
	pages = "1--67",
	publisher = "The Institute of Mathematical Statistics",
	title = "Multivariate Adaptive Regression Splines",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1214/aos/1176347963",
	volume = "19",
	year = "1991"
}


@article{mccradshock10,
	title = "Anti-diffusive radiation flow in the cooling layer of a radiating shock ",
	journal = "Journal of Quantitative Spectroscopy and Radiative Transfer ",
	volume = "111",
	number = "14",
	pages = "2095 - 2105",
	year = "2010",
	note = "",
	issn = "0022-4073",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.jqsrt.2010.05.013",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__www.sciencedirect.com_science_article_pii_S0022407310001822&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=-yg7uEjlJnQdvFrVcrDG-dw2rFND6A4spkIrgue7DUQ&e= ",
	author = "Ryan G. McClarren and R. Paul Drake",
	keywords = "Radiative transfer",
	keywords = "Eddington approximation",
	keywords = "Diffusion methods "
}

@article{mccfpn09,
	title = "Simulating radiative transfer with filtered spherical harmonics ",
	journal = "Physics Letters A ",
	volume = "374",
	number = "22",
	pages = "2290 - 2296",
	year = "2010",
	note = "",
	issn = "0375-9601",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/j.physleta.2010.02.041",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__www.sciencedirect.com_science_article_pii_S0375960110002021&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=iaeehuMn_iiTwpkAEwweuaM37Bix6okA_k9UR1lGNts&e= ",
	author = "Ryan G. McClarren and Cory D. Hauck",
	keywords = "Radiation transport",
	keywords = "High eneR. G.y density physics",
	keywords = "Kinetic equations",
	keywords = "Spherical harmonics method "
}



@article{levermoredn,
	author = {Matthias Sch\"{a}fer and Martin Frank and C. David Levermore},
	title = {{Diffusive Corrections to PN Approximations}},
	journal = {Multiscale Modeling \& Simulation},
	volume = {9},
	number = {1},
	pages = {1-28},
	year = {2011},
	doi = {10.1137/090764542}	
}

@CONFERENCE{p3qs,
	author={Oh, K. S. and Holloway, J. P.},
	title={{A Quasi-static Closure for 3rd Order Spherical Harmonics Time-Dependent Radiation Transport in 2-D}},
	journal={American Nuclear Society - International Conference on Mathematics, Computational Methods and Reactor Physics 2009, M\& C 2009},
	year={2009},
	volume={3},
	pages={1938-1948},
	note={cited By 0},
	url={https://urldefense.proofpoint.com/v2/url?u=http-3A__www.scopus.com_inward_record.url-3Feid-3D2-2Ds2.0-2D74549196287-26partnerID-3D40-26md5-3D067624efc28e6ab8fcd497d7c581617a&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=_Vbk27qMiDqEaQvmJL6RqZRl08FqfhritqCMuiQiGeg&e= },
	document_type={Conference Paper},
	source={Scopus},
}

@CONFERENCE{ahrens_fpn,
	author={Cory Ahrens and Simon Merton},
	title={{An Improved Filtered Spherical Harmonic Method for Transport Calculations}},
	journal={American Nuclear Society - International Conference on Mathematics, Computational Methods and Reactor Physics 2009, M\& C 2013},
	year={2013},
	document_type={Conference Paper},
	source={Scopus},
}

@article{brunnerentropy,
	title = "One-dimensional {Riemann} solvers and the maximum entropy closure ",
	journal = "Journal of Quantitative Spectroscopy and Radiative Transfer ",
	volume = "69",
	number = "5",
	pages = "543 - 566",
	year = "2001",
	note = "",
	issn = "0022-4073",
	doi = "https://urldefense.proofpoint.com/v2/url?u=http-3A__dx.doi.oR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=Bd7WDKMxMMK9PIRzufS_y-BKHCwX9TzwA_LAOKYb_qs&e= . G./10.1016/S0022-4073(00)00099-6",
	url = "https://urldefense.proofpoint.com/v2/url?u=http-3A__www.sciencedirect.com_science_article_pii_S0022407300000996&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=RA5nrsCg0Nvo45EzkxR_cWFtyKRPL7WnekXtsp3PiAk&e= ",
	author = "Thomas A. Brunner and James Paul Holloway",
	keywords = "Maximum entropy closure",
	keywords = "Riemann solver",
	keywords = "Time-dependent transport "
}

@article{coryentropy,
	title={High-order entropy-based closures for linear transport in slab geometry},
	author={Hauck, Cory D},
	journal={Commun. Math. Sci},
	volume={9},
	number={1},
	pages={187--205},
	year={2011}
}

@misc{legendrerecur,
	author   = {Weisstein, Eric W.},
	title    = {Legendre Polynomial. {From MathWorld---A Wolfram Web Resource}},
	url      = {\url{https://urldefense.proofpoint.com/v2/url?u=http-3A__mathworld.wolfram.com_LegendrePolynomial.html&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=vHfcu98aynooirYRz5Yi1InxyNLuN8ZONP909EAtV_E&e= }},
	note     = {Last visited on 13/4/2012},
}


@CONFERENCE{petermc,
	author={Maginot, Peter and Morel, Jim and Ragusa J. E.an},
	title={A Positive Non-Linear Closure for the Sn Equations with Linear-Discontinous Spatial Differencing},
	journal={American Nuclear Society - International Conference on Mathematics, Computational Methods and Reactor Physics 2009, M and C 2009},
	place={Saratoga Springs, New York, United States},
	year={2009},
	volume={3},
	pages={1938-1948}, %note={cited By 0},
	document_type={Conference Paper},
	source={Scopus},
}

@conference{clifmc,
	author={Drumm, Clif},
	title={Spherical Harmonics ({P$_n$}) Methods In The Sceptre Radiation Transport Code},
	booktitle={ANS MC2015 - Joint International Conference on Mathematics and Computation (M\&C), Supercomputing in Nuclear Applications (SNA) and the Monte Carlo (MC) Method},
	note={Nashville, TN, United States},
	year={2015},
	document_type={Conference Paper},
	source={Scopus},
}

@conference{morel_holo,
	author={Jacob R. Peterson and Hans R. Hammer and Jim E. Morel and Jean C. Ragusa and Yaqi Wang},
	title={{Conservative Nonlinear Diffusion Acceleration Applied to the Unweighted Least-squares Transport Equation in MOOSE}},
	booktitle={ANS MC2015 - Joint International Conference on Mathematics and Computation (M\&C), Supercomputing in Nuclear Applications (SNA) and the Monte Carlo (MC) Method},
	note={Nashville, TN, United States},
	year={2015},
	document_type={Conference Paper},
}

@ARTICLE{guermond_l1,
	author = {J. L. Guermond},
	title = {A Finite Element Technique for Solving First Order PDEs in ${L}_p$},
	journal = {SIAM J. Numer. Anal},
	volume = {42},
	number = {2},
	year = {2004},
	pages = {714-737},
}

@article{lowrie_l1,
	title = "On the Numerical Solution of Conservation Laws by Minimizing Residuals ",
	journal = "Journal of Computational Physics ",
	volume = "113",
	number = "2",
	pages = "304 - 308",
	year = "1994",
	author = {R.B. Lowrie and P.L. Roe}
	
}

@article{bnjiang_l1,
	title = "Non-oscillatory and Non-diffusive Solution of Convection Problems by the Iteratively Reweighted  Least-Square Finite Element Method ",
	journal = "Journal of Computational Physics ",
	volume = "105",
	pages = "108 - 121",
	year = "1993",
	author = {B.N. Jiang}
}

@article{reed_1971, 
	title={New Difference Schemes For The Neutron Transport Equation}, 
	journal={Nucl. Sci. Eng. 46:  No. 2, 309-14}, author={Reed, W.H.}, year={1971}}

@article{dealii82,
	title = {The \texttt{deal.II} Library, Version 8.2},
	author = {W. Bangerth and T. Heister and L. Heltai
	and G. Kanschat and M. Kronbichler
	and M. Maier and B. Turcksin
	and T. D. Young},
	journal = {Archive of Numerical Software},
	volume = 3,
	year = {2015},
}

%% This BibTeX bibliography file was created using BibDesk.
%% https://urldefense.proofpoint.com/v2/url?u=http-3A__bibdesk.sourcefoR&d=BQIGaQ&c=54IZrppPQZKX9mLzcGdPfFD1hxrcB__aEkJFOKJFd00&r=vagGGoKMDjEcmkK-jVg_tYrRoZRPgGrNDN65NN6Hyl0&m=r0JTkL_p2jrqQlWicJQiKr6WX7Yoya9bfF62_e5jGgo&s=XP8UuvJWF1xL_35RfwLInaXe_DvcUF4h3OWCv8KMJJ4&e= . G.e.net/


%% Created for Seth Johnson at 2010-01-15 15:01:56 -0500 


%% Saved with string encoding Unicode (UTF-8) 



@article{Lar2008,
	Author = {Larsen, Edward W. and Wollaber, Allan B.},
	Date-Added = {2010-01-15 15:01:35 -0500},
	Date-Modified = {2010-01-15 15:01:35 -0500},
	Journal = {Nuclear Science and Engineering},
	Keywords = {SN},
	Number = {3},
	Pages = {267--283},
	Title = {A Quantitative Theory of Angular Truncation Errors in Three-Dimensional {$S_N$} Calculations},
	Volume = {160},
	Year = {2008}}

@article{park-nda,
	Author = {D. A. Knoll and H. Park and K. Smith},
	Journal = {Nuclear Science and Engineering},
	Keywords = {SN},
	Number = {2},
	Pages = {122--132},
	Title = {Application of the Jacobian-Free Newton-Krylov Method to Nonlinear Acceleration of Transport Source Iteration in Slab Geometry},
	Volume = {167},
	Year = {2011}}

@article{ls-60s,
	Author = {B. A. Finlayson and L. E. Scriven},
	Journal = {Applied Mathematics Reviews},
	Number = {9},
	Pages = {735--748},
	Title = {The Method of Weighted Residuals--A Review},
	Volume = {19},
	Year = {1966}}

@article{ls-70s,
	Author = {E. D. Eason},
	Journal = {INTERNATIONAL JOURNAL FOR NUMERICAL METHODS IN ENGINEERING},
	Pages = {1021--1046},
	Title = {A REVIEW OF LEAST-SQUARES METHODS FOR SOLVING PARTIAL DIFFERENTIAL EQUATIONS},
	Volume = {10},
	Year = {1976}}

@article{ls-80s,
	Author = { Liable, J. and Pinder, G.},
	Journal = {Numer. Methods Partial Differential Equations},
	Pages = {347--361},
	Title = {Least-squares collocation solution of differential equations on irregularly shaped domains using orthogonal meshes},
	Volume = {5},
	Year = {1989}}

@techreport{Car1953,
	Author = {Carlson, Bengt G.},
	Date-Added = {2010-01-15 14:53:00 -0500},
	Date-Modified = {2010-01-15 14:53:00 -0500},
	Institution = {Los Alamos Scientific Laboratory},
	Number = {LA-1599},
	Title = {Solution of the Transport Equation by {S$_n$} Approximations},
	Year = {1953}}

@techreport{ganapol,
	author={Ganapol, B. D. and Baker, R. S.  and Dahl, J. A. and Alcouffe, Raymond E.},
	Institution = {Los Alamos National Laboratory},
	Number = {LA-UR--01-1854},
	Title = {Homogeneous Infinite Media Time-Dependent Analytical Benchmarks},
	Year = {2001}}

@techreport{brunner_app_rad_trans,
	Author = {Brunner, Thomas A.},
	Institution = {Sandia National Laboratory},
	Number = {SAND2002-1778},
	Title = {{Forms of Approximate Radiation Transport}},
	Year = {2002}}

@book{Kno2000,
	Author = {Knoll, Glenn F.},
	Date-Added = {2010-01-15 14:52:06 -0500},
	Date-Modified = {2010-01-15 14:52:06 -0500},
	Edition = {3rd},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Radiation Detection and Measurement},
	Year = {2000}}

@article{Pul2010,
	Author = {Pullum, Geoffrey K.},
	Journal = {English Today},
	Number = {2},
	Pages = {34--44},
	Title = {The Land of the Free and \emph{The Elements of Style}},
	Volume = {26},
	Year = {2010}}

@book{Str2000,
	Author = {Strunk, W. and White, E.B.},
	Edition = {4},
	Publisher = {New York: Allyn and Bacon},
	Title = {The Elements of Style},
	Year = {2000}}

@book{lewis1993
    author = {Warren F. Miller and Elmer E. Lewis},
    edition = {1},
    year = {1993},
    publisher = {{American Nuclear Society}},
    title = {{Computational Methods of Neutron Transport}}
}


